AI Hospital: Benchmarking Large Language Models in a Multi-agent Medical Interaction Simulator

Artificial intelligence has significantly advanced healthcare, particularly through large language models (LLMs) that excel in medical question answering benchmarks. However, their real-world clinical application remains limited due to the complexities of doctor-patient interactions. To address this, we introduce \textbf{AI Hospital}, a multi-agent framework simulating dynamic medical interactions between \emph{Doctor} as player and NPCs including \emph{Patient}, \emph{Examiner}, \emph{Chief Physician}. This setup allows for realistic assessments of LLMs in clinical scenarios. We develop the Multi-View Medical Evaluation (MVME) benchmark, utilizing high-quality Chinese medical records and NPCs to evaluate LLMs' performance in symptom collection, examination recommendations, and diagnoses. Additionally, a dispute resolution collaborative mechanism is proposed to enhance diagnostic accuracy through iterative discussions. Despite improvements, current LLMs exhibit significant performance gaps in multi-turn interactions compared to one-step approaches. Our findings highlight the need for further research to bridge these gaps and improve LLMs' clinical diagnostic capabilities. Our data, code, and experimental results are all open-sourced at \url{https://github.com/LibertFan/AI_Hospital}.

==> Section/Tables/Department_Distribution.tex <==
\begin{table}
    \caption{Departments distribution of the collected medical records.}
    \label{table:department_distribution}
    \vspace{2mm}
    \centering
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{cc}
        \toprule
        Department & \# \\
        \midrule
        Surgery & 180 \\
        Internal Medicine & 153 \\
        Obstetrics and Gynecology &94  \\
        Pediatrics &29  \\
        Otorhinolaryngology &23  \\
        Others & 27 \\
        \bottomrule
    \end{tabular}
    }
\end{table}
% 外科病例': 227, '内科病例': 206, '妇产科病例': 94, '耳鼻咽喉科病例': 29, '儿科病例': 26
% '外科病例': 180, '内科病例': 153, '妇产科病例': 94, '儿科病例': 29, '耳鼻咽喉科病例': 23, '护理科病例': 14


==> Section/Tables/Error_Types.tex <==
\begin{table}[!th]
    \caption{Classification and statistics of misdiagnoses (1 point) of the intern doctor powered by GPT-4.}
    \label{table:error_types}
    \vspace{2mm}
    \centering
    %\resizebox{0.39\textwidth}{!}{
    \begin{tabular}{cc}
        \toprule
        Error Type & \# \\
        \midrule
        Omission of auxiliary examinations & 99 \\
        Exclusive focus on complications & 52 \\
        Erroneous judgment & 68 \\
        \bottomrule
    \end{tabular}
    %}
\end{table}

==> Section/Tables/LLM_Performance.tex <==
\begin{table*}[ht]
% \small 
\centering
\setlength\tabcolsep{13pt} % 列间距
\caption{LLM-based Evaluation with Reference in Medical Consultation. GPT-4$^{*}$ in One-Step is the upper bound.} % One Step refers to a process where a diagnosis is directly generated in one step based on a patient's symptoms and medical examination results. The initial two intern doctors are empowered by GPT-3.5 and GPT-4 for interactive consultation, and the subsequent addition in 3 doctors is using Wenxin.}
% 2 doctors are GPT-4 and GPT-3.5. 3 doctors are GPT-4, GPT-3.5 and Wenxin 4.0.}
\begin{tabular}{l|cccc}
\toprule
%\textbf{LLM} &\textbf{Diagnosis} &\textbf{Basis}  &\textbf{Treatment} \\ 
\textbf{LLM} &Diagnostic Results  &Rationales &Treatment Plan \\
\midrule
&\multicolumn{3}{c}{Interaction} \\
\midrule
DISC-MedLLM (13B) &$1.587 \pm 0.063$ &$1.424 \pm 0.058$ &$1.172 \pm 0.036$ \\ 
Baichuan (13B) &$1.746 \pm 0.073$ &$1.715 \pm 0.069$ &$1.343 \pm 0.053$ \\ 
HuatuoGPT-II (13B) &$1.884 \pm 0.072$ &$1.899 \pm 0.072$ &$1.529 \pm 0.064$ \\ 
HuatuoGPT-II (34B) &$2.096 \pm 0.078$ &$2.112 \pm 0.078$ &$1.826 \pm 0.078$ \\
Qwen &$2.159 \pm 0.077 $ &$2.222 \pm 0.076$ &$1.908 \pm 0.076$\\ 
GPT-3.5 &$2.133 \pm 0.072$ & $2.195 \pm 0.069$ & $1.648 \pm 0.067$ \\ 
Wenxin  & $2.170\pm0.072$ & $2.178\pm0.069$ &$1.836\pm0.067$\\ 
GPT-4 & $2.237\pm0.070$ & $2.300\pm0.069$ &$1.998\pm0.072$\\ 
\midrule
&\multicolumn{3}{c}{Collaboration} \\
\midrule
2 Doctors  & $2.481\pm0.065$ & $2.482\pm0.063$ &$2.146\pm0.066$\\
2 Doctors w/o DR & $2.403\pm0.067$ & $2.429\pm0.062$ &$2.066\pm0.067$\\ 
3 Doctors & $2.508\pm0.067$ & $2.538\pm0.062$ &$2.207\pm0.066$\\ 
\midrule
&\multicolumn{3}{c}{One-Step} \\
\midrule
GPT-4$^{*}$  & $3.110\pm 0.025$ & $3.008\pm 0.018$ &$2.657\pm 0.046$\\ 
\bottomrule
\end{tabular}
\label{table:llm_evaluation}
\end{table*}
% mean: 3.110, ci: (3.085, 3.134), range: 0.025
% mean: 3.008, ci: (2.990, 3.026), range: 0.018
% mean: 2.658, ci: (2.610, 2.704), range: 0.046



==> Section/Tables/Link_based_Performace.tex <==
\begin{table}[ht]
% \small 
\centering
\caption{MVME: Link-based evaluation of diagnostic results in clinical consultation.}
\label{table:link_evaluation}
\vspace{2mm}
% \setlength\tabcolsep{13pt} % 列间距
% 2 doctors are GPT-4 and GPT-3.5. 3 doctors are GPT-4, GPT-3.5 and Wenxin 4.0.}
% \resizebox{0.65\textwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
% {LLM} 
&{\#} &{R}  &{P} &{F1} \\ 
\midrule
&\multicolumn{4}{c}{Interaction} \\
\midrule
Baichuan (13B) &1.58 &10.21 &23.79 &14.28 \\
HuatuoGPT-II (13B) &1.72 &12.76 &24.84 &16.85 \\
HuatuoGPT-II (34B) & 1.86 &17.48& 30.95 & 22.34 \\
GPT-3.5 &1.81 &19.19& 37.39 & 25.37  \\
Wenxin-4.0 &2.50 &22.03& 31.44 & 25.91 \\
Qwen-Max & 1.77 &\textbf{22.42} & 43.38 & 29.56 \\ 
GPT-4 &1.52 &21.64&\textbf{50.26} & \textbf{30.26} \\
\midrule
&\multicolumn{4}{c}{Collaboration} \\
\midrule
2 Doctors w/o DR &2.37 &28.44 &41.45 &33.74 \\
2 Doctors  &2.41 &29.51 &\textbf{43.62} &35.21 \\
3 Doctors &3.20 &\textbf{36.54} &39.58 &\textbf{38.00} \\
\midrule
&\multicolumn{4}{c}{One-Step} \\
\midrule
GPT-4$^{*}$  &2.30 &38.90 &58.97 &46.88 \\
% \midrule
% &\multicolumn{3}{c}{One Step} \\
% \midrule
% GPT-4  & $3.110\pm 0$ & $3.008\pm 0$ &$2.657\pm 0$\\ 
% \midrule
% &\multicolumn{3}{c}{Collaboration} \\
% \midrule
% 2 Doctors  & $2.41\pm0.067$ & $2.509\pm0.062$ &$2.146\pm0.067$\\ 
% \quad w/o DR & $2。37\pm0.067$ & $2.509\pm0.062$ &$2.146\pm0.067$\\ 
% 3 Doctors & $2.483\pm0.067$ & $2.509\pm0.062$ &$2.146\pm0.067$\\ 
\bottomrule
\end{tabular}
% }
\end{table}
%  1.50       |    7.34    |     18.84     | 10.57  |   24.86
% GPT-3.5-Turbo-1118&     500  &1.81 &19.19& 37.39 & 25.37  
% GPT-4-1122    &     505  & 1.52 &21.64& 50.26 & 30.26 
% WenXin-1120    &     408  & 2.50 &22.03& 31.44 & 25.91 
% Qwen200B     &     452  & 1.77 &22.42& 43.38 & 29.56 
% HuatuoGPT2_34B  &     248  & 1.86 &17.48& 30.95 & 22.34 
% 3.20       |   36.54    |     39.58     | 38.00
%2.30       |   38.90    |     58.97     | 46.88 

==> Section/Tables/Medical_Records.tex <==
\begin{table*}[ht]
% \small 
\centering
\setlength\tabcolsep{13pt} % 列间距
\caption{Details of Medical Records.}
\begin{tabular}{l|c}
\toprule
 & \\ 
\midrule
Item & Explanation \\
\midrule
[General Information]& \\ % This section includes basic patient information, such as name, sex, age, occupation, address, and so on.
[Chief Complaint]& \\ % The main reason the patient is seeking medical attention or the most significant and prominent symptoms, typically as described by the patient themselves.
[Present Illness History]& \\ % Describes the onset, course, changes, and related symptoms of the patient's current illness in detail.
[Past Medical History]& \\ % The patient's past health conditions, including previous diseases, injuries, surgeries, allergies, etc.
[Personal History]& \\ % Relevant information about the patient's lifestyle habits, living environment, occupation, and family medical history.
[Physical Examination]& \\ % The results of the physical examination conducted by the doctor, which usually includes vital signs and the examination results of various systems.
[Auxiliary Examination]& \\ % Results of examinations such as X-rays, blood tests, ultrasounds, MRIs, etc.
[Preliminary Judgment]& \\ % Based on the above information, the doctor's initial diagnosis or assessment of the condition.
[Basis for Judgment]& \\ % The evidence or reasons relied upon for the preliminary judgment made.
[Differential Diagnosis]& \\ % For certain diseases, there may be several similar conditions; this section lists and analyzes these possibilities.
[Diagnostic Process]& \\ % Describes the entire process from diagnosis to treatment, including the medical measures taken and the patient's response.
[Diagnosis]& \\ % The name or state of the disease determined after diagnosis.
[Analysis and Summary]& \\ % A comprehensive analysis and commentary on the entire case, sometimes including suggestions for the patient's treatment and prognosis.
\bottomrule
\end{tabular}
\label{llm_evaluation_table}
\end{table*}

==> Section/Tables/Prompt_Evaluate.tex <==
\begin{table*}[h]
\begin{tcolorbox}[colback=blue!5!white,colframe=black,width=1.0\textwidth,title={Prompt for Medical Director to Evaluate}]
\small
\begin{CJK}{UTF8}{gbsn}
\textbf{System Message} 
\vspace{3pt} \\
你是资深的医学专家。你需要根据专家诊断报告来判断实习医生诊断报告中的三部分（诊断结果、诊断依据和治疗方案）的正确性。
\vspace{3pt} \\
评价过程中请参考下面的细则，判断每个部分实习医生与专家之间的一致性。
\vspace{2pt} \\
1. 诊断结果\\
\ \ (A) 完全一致，诊断正确\\
\quad (B) 相当部分一致，诊断基本正确\\
\quad (C) 小部分一致，诊断存在错误\\
\quad (D) 完全不一致，诊断完全错误
\vspace{2pt} \\
2. 诊断依据\\
\quad (A) 完全一致 \\
\quad (B) 相当部分一致 \\
\quad (C) 小部分一致 \\
\quad  (D) 完全不一致
\vspace{2pt} \\
3. 治疗方案\\
\quad (A) 完全一致\\
\quad (B) 相当部分一致\\
\quad (C) 小部分一致\\
\quad (D) 完全不一致
\vspace{3pt} \\
按照下面的格式输出结果
\vspace{2pt} \\
\# 诊断结果\\
分析: xx\\
选项: xx
\vspace{2pt} \\
\# 诊断依据 \\
分析: xx \\
选项: xx
\vspace{2pt} \\
\# 治疗方案 \\
分析: xx \\
选项: xx 
\vspace{3pt} \\
(1)请侧重医学答案的事实内容，不需关注风格、语法、标点和无关医学的内容。 \\
(2) 请你充分利用医学知识，分析并判断每个点的重要性，再做评价。\\
(3) 注意诊断结果、诊断依据和治疗方案三者之间的承接关系。
\vspace{5pt} \\
\textbf{User}
\vspace{3pt} \\
\# 专家的诊断报告 \\
\{Diagnosis and Treatment in \S\ref{section_medical_records}\} \\
\# 实习医生的诊断报告 \\
\{实习医生的诊断报告\}
\end{CJK}
\end{tcolorbox}
\caption{The original Chinese prompt for medical director to evaluate.}
\label{agent:evaluate:zh}
\end{table*}

% As an experienced medical expert, your task is to evaluate the accuracy of three components in an intern doctor's diagnostic report—diagnosis, diagnostic rationale, and treatment plan—by comparing it with the medical director's report.

% During the evaluation, adhere to these guidelines to assess the congruence between the intern doctor's and the medical director's findings in each component:

\begin{table*}[h]
\begin{tcolorbox}[colback=blue!5!white,colframe=black,width=1.0\textwidth,title={Prompt for Medical Director to Evaluate}]
\small
You are an experienced medical expert. Your task is to evaluate the accuracy of three components in an intern doctor's diagnostic report—diagnostic result, diagnostic rationale, and treatment plan—by comparing it with the medical director's report.
\vspace{3pt} \\
During the evaluation process, please refer to the following guidelines to judge the consistency between the intern doctor's and the medical director's findings in each component:
\vspace{2pt} \\
1. Diagnosis Result \\
   (A) Completely consistent, correct diagnosis \\
   (B) Largely consistent, basically correct diagnosis \\
   (C) Partially consistent, diagnosis contains errors \\
   (D) Completely inconsistent, completely incorrect diagnosis 
\vspace{2pt} \\
2. Diagnostic Rationale \\
   (A) Completely consistent \\
   (B) Largely consistent \\
   (C) Partially consistent \\
   (D) Completely inconsistent 
\vspace{2pt} \\
3. Treatment Plan \\
   (A) Completely consistent \\
   (B) Largely consistent \\
   (C) Partially consistent \\
   (D) Completely inconsistent 
\vspace{3pt} \\
Please output the results in the following format:
\vspace{2pt} \\
\# Diagnosis Result \\
Analysis: xx \\
Option: xx 
\vspace{2pt} \\
\# Diagnostic Rationale \\
Analysis: xx \\
Option: xx 
\vspace{2pt} \\
\# Treatment Plan \\
Analysis: xx \\
Option: xx 
\vspace{3pt} \\
(1) Please focus on the factual content of the medical answers, without concern for style, grammar, punctuation, and content unrelated to medicine. \\
(2) Please make full use of your medical knowledge to analyze and judge the importance of each point before evaluating. \\
(3) Pay attention to the continuity among the diagnosis result, diagnostic basis, and treatment plan. 
\vspace{5pt} \\
\textbf{User}
\vspace{3pt} \\
\# Diagnostic Report of Medical Director\\
\{Diagnosis and Treatment in Section \ref{section_medical_records}\} \\
\# Diagnostic Report of Intern Doctor \\
\{Diagnostic Report of the Intern Doctor\}
\end{tcolorbox}
\caption{The translated English prompt for medical director to evaluate.}
\label{agent:evaluate:en}
\end{table*}
